Optimal Persistent Monitoring of Mobile Targets in One Dimension

This work shows the existence of optimal control laws for persistent monitoring of mobile targets in a one-dimensional mission space and derives explicit solutions. The underlying performance metric consists of minimizing the total uncertainty accumulated over a finite mission time. We first demonstrate that the corresponding optimal control problem can be reduced to a finite-dimensional optimization problem, and then establish existence of an optimal solution. Motivated by this result, we construct a parametric reformulation for which an event based gradient descent method is utilized with the goal of deriving (locally optimal) solutions. We additionally provide a more practical parameterization that has attractive properties such as simplicity, flexibility, and robustness. Both parameterizations are validated through simulation.

==> setup/tikz_setup.tex <==

%% Tikz
\usepackage{tikz}
\usetikzlibrary{positioning, arrows, calc, arrows.meta}

\tikzset{
	%Define standard arrow tip
	>=stealth',
	%Define style for different line styles
	help lines/.style={dashed, thick},
	axis/.style={<->},
	important line/.style={thick},
	connection/.style={thick, dotted},
}

%% PGF plots
\usepackage{pgfplots, pgfplotstable}
\pgfplotsset{compat=1.16}
\newlength\fheight
\newlength\fwidth
\setlength\fheight{4cm}
\setlength\fwidth{6cm}

